Reaching Goals is Hard: Settling the Sample Complexity of the Stochastic Shortest Path

We study the sample complexity of learning an $\epsilon$-optimal policy in the Stochastic Shortest Path (SSP) problem. We first derive sample complexity bounds when the learner has access to a generative model. We show that there exists a worst-case SSP instance with $S$ states, $A$ actions, minimum cost $c_{\min}$, and maximum expected cost of the optimal policy over all states $B_{\star}$, where any algorithm requires at least $\Omega(SAB_{\star}^3/(c_{\min}\epsilon^2))$ samples to return an $\epsilon$-optimal policy with high probability. Surprisingly, this implies that whenever $c_{\min}=0$ an SSP problem may not be learnable, thus revealing that learning in SSPs is strictly harder than in the finite-horizon and discounted settings. We complement this result with lower bounds when prior knowledge of the hitting time of the optimal policy is available and when we restrict optimality by competing against policies with bounded hitting time. Finally, we design an algorithm with matching upper bounds in these cases. This settles the sample complexity of learning $\epsilon$-optimal polices in SSP with generative models. We also initiate the study of learning $\epsilon$-optimal policies without access to a generative model (i.e., the so-called best-policy identification problem), and show that sample-efficient learning is impossible in general. On the other hand, efficient learning can be made possible if we assume the agent can directly reach the goal state from any state by paying a fixed cost. We then establish the first upper and lower bounds under this assumption. Finally, using similar analytic tools, we prove that horizon-free regret is impossible in SSPs under general costs, resolving an open problem in (Tarbouriech et al., 2021c).

==> hf.tex <==
%In this section, we show that our techniques developed in previous sections also resolve an open question in~\cite{tarbouriech2021stochastic}.
%Specifically, we show that in regret minimization, a worst-case dependency on the hitting time of the optimal policy is indeed unavoidable without any prior knowledge.

Recently \cite{zhang2022horizon} show that in finite-horizon MDPs it is possible to achieve a horizon-free regret bound with no horizon dependency even in logarithmic terms.
For SSPs, \cite{tarbouriech2021stochastic} achieves a nearly horizon-free regret bound $R_K\lesssim\B\sqrt{SAK}\ln\frac{1}{\lambda} + \B S^2A + \lambda\T K$ for any given $\lambda>0$ in $K$ episodes without knowledge of $\T$, where regret $R_K=\sumk(\sum_{i=1}^{I_k}c(s^k_i,a^k_i)-\optV(\sinit))$, and $R_K=\infty$ if $I_k=\infty$ for some $k$.
% \matteo{There is an additional $K$ in the low order term\lc{I do not understand this comment actually, you mean it should be $\lambda\T$ or $\lambda\T K^2$?} I was thinking about $\lambda\T$ with $\lambda$ tuned to be $\T$ with prior knowledge but equivalently you can say that $\lambda = poly(K) \T^{-1}$\lc{I think what I wrote here is the original form. If we set $c'(s,a)=\max\{\lambda,c(s, a)\}$. Then the bias term is $\lambda\T K$.} }
If a prior knowledge $\uT=\T$ is available, their result is horizon-free.
A natural question to ask is whether horizon-free regret is possible in SSPs without prior knowledge.
We show that this is actually impossible. % without any prior knowledge.
%Horizon-free regret bound is shown to be possible in finite-horizon MDPs~\citep{zhang2022horizon}.
%We prove a negative result stating that horizon-free regret bound is impossible in SSP.

\begin{definition}
    \label{def:hf}
    %Consider two functions $c_1, c_2: \fR_+\times \fN_+\times\fN_+\times(0,1)\times\fN_+\rightarrow \fR_+$, such that for $i\in\{1, 2\}$, $c_i(\B, S, A, \delta, K)$ has poly-logarithmic dependency on $K$.
    We say an algorithm is $(c_1, c_2)$-horizon-free if when it takes number of episodes $K\geq 1$, failure probability $\delta\in(0,1)$, and an SSP instance $\calM$ with parameters $\B$, $S$, $A$ as input, it achieves $R_K\leq c_1(\B, S, A, K, \delta)\sqrt{K}+c_2(\B, S, A, K, \delta)$ on $\calM$ with probability at least $1-\delta$,
    %where $c_1, c_2: \fR_+\times \fN_+\times\fN_+\times(0,1)\times\fN_+\rightarrow \fR_+$ and $c_i(\B, S, A, K, \delta)$ has poly-logarithmic dependency on $K$ for $i\in\{1, 2\}$ (no dependency on $\T$ and $\frac{1}{\cmin}$).
    where $c_1$, $c_2$ are functions of $\B$, $S$, $A$, $K$, $\delta$ that have poly-logarithmic dependency on $K$ (no dependency on $\T$ and $\frac{1}{\cmin}$).
\end{definition}

\begin{theorem}
    \label{thm:hf}
    For any $c_1,c_2$ that are functions of $\B$, $S$, $A$, $K$, $\delta$, and have poly-logarithmic dependency on $K$, there is no $(c_1, c_2)$-horizon-free algorithm.
    %There is no $(c_1, c_2, K, \delta)$-horizon-free algorithm under general costs, for any $c_1,c_2>0$, $K\geq 1$, and $\delta\in(0, \frac{1}{8})$ such that $c_1\sqrt{K}+c_2 < \frac{K}{2}$ for all $\B\leq 1$.
\end{theorem}
Details are deferred to \pref{app:hf}.
Finally, note that in regret minimization the regret bound can scale with $\T$ even without knowledge of $\T$, while in sample complexity we cannot (\pref{thm:lower.bound.eps.T}). Therefore, computing $\epsilon$-optimal policy in SSP is in some sense more difficult than regret minimization.

